Advancing On-Device Neural Network Training with TinyPropv2: Dynamic, Sparse, and Efficient Backpropagation

This study introduces TinyPropv2, an innovative algorithm optimized for on-device learning in deep neural networks, specifically designed for low-power microcontroller units. TinyPropv2 refines sparse backpropagation by dynamically adjusting the level of sparsity, including the ability to selectively skip training steps. This feature significantly lowers computational effort without substantially compromising accuracy. Our comprehensive evaluation across diverse datasets CIFAR 10, CIFAR100, Flower, Food, Speech Command, MNIST, HAR, and DCASE2020 reveals that TinyPropv2 achieves near-parity with full training methods, with an average accuracy drop of only around 1 percent in most cases. For instance, against full training, TinyPropv2's accuracy drop is minimal, for example, only 0.82 percent on CIFAR 10 and 1.07 percent on CIFAR100. In terms of computational effort, TinyPropv2 shows a marked reduction, requiring as little as 10 percent of the computational effort needed for full training in some scenarios, and consistently outperforms other sparse training methodologies. These findings underscore TinyPropv2's capacity to efficiently manage computational resources while maintaining high accuracy, positioning it as an advantageous solution for advanced embedded device applications in the IoT ecosystem.

==> 5hyperparameter.tex <==

\section{hyperparameter selection}
We have introduced new hyperparameters with TinyProp to better control the available resources of the embedded systems in the training. In this chapter, we would like to explain how the hyperparameters should be chosen in order to adapt the algorithm to the target device in the best possible way.

We have conducted several experiments with different sets of hyperparameters. The results with the different hyperparameter settings are shown in Table \ref{tab:anoresult} and \ref{tab:mnistresult}.
Each of these experiments was performed 100 times with random initializations and we have taken the average of the results.
The result was that the exact settings are not that important to get a good result. However, the more we allow to train, the better the result. 
The most important hyperparameter is $S_{max}$. With the help of $S_{max}$ we can control whether a net is trained from the scratch or whether the net is fine-tuned. 
A recommendation drawn from the experience of the experiments is as follows:


\begin{table}[!h]\centering
\caption{TinyProp hyperparameter}
\label{tab:hyperparasel}
\begin{tabular}{llll}
                      & $S_{max}$ & $S_{min}$ & $\zeta$ \\
                      \hline
Training from scratch & 0.8  & 0.1  & 0.9  \\
Fine-Tune DNN       & 0.4  & 0.1  & 0.9
\end{tabular}
\end{table}


